Learning Causal Models from Conditional Moment Restrictions by Importance Weighting

We consider learning causal relationships under conditional moment restrictions. Unlike causal inference under unconditional moment restrictions, conditional moment restrictions pose serious challenges for causal inference, especially in high-dimensional settings. To address this issue, we propose a method that transforms conditional moment restrictions to unconditional moment restrictions through importance weighting, using a conditional density ratio estimator. Using this transformation, we successfully estimate nonparametric functions defined under conditional moment restrictions. Our proposed framework is general and can be applied to a wide range of methods, including neural networks. We analyze the estimation error, providing theoretical support for our proposed method. In experiments, we confirm the soundness of our proposed method.

==> IWMM (1)/def.tex <==
\usepackage{bm}
\usepackage{bbm}
\usepackage{multicol,multirow}
\usepackage{comment}
\usepackage{booktabs}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\Ie}{\textit{I.e.}}
\newcommand{\Eg}{\textit{E.g.}}
\usepackage{enumerate}   
\usepackage{amsmath}
\def \dr {\mathrm{DR}}
\usepackage{wrapfig}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

\usepackage{appendix}
\usepackage{amssymb}


\newcommand{\lbl}[1]{\label{#1}{\ensuremath{^{\fbox{\tiny\upshape#1}}}}}
\renewcommand{\lbl}[1]{\label{#1}}

\usepackage{amsthm}
\usepackage{hyperref}
\usepackage[capitalise]{cleveref}
\Crefname{assumption}{Assumption}{Assumptions}


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

%
%
\DeclareMathOperator*{\plim}{plim}
\newcommand{\indep}{ \stackrel{indep}{\sim} }
\newcommand{\iid}{ \stackrel{i.i.}{\sim} }
\newcommand{\bx}{\mathbf{x}}
\newcommand{\btau}{\mathbf{\tau}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bpi}{\pmb{\pi}}
\newcommand{\bh}{\mathbf{\pi}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\smallo}{{\scriptscriptstyle\mathcal{O}}} %
\newcommand{\bo}{\mathbf{0}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bG}{\mathbb{G}}
\def\Holder{{H\"{o}lder}}
\newcommand{\bu}{\mathbf{u}}
\def\Cramer{Cram\'{e}r}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\nhs}{n^{\mathrm{hst}}}
\newcommand{\fix}{\mathrm{fix}}
\newcommand{\nev}{n^{\mathrm{evl}}}
\newcommand{\EB}{\mathrm{EB}}
\newcommand{\para}{\mathrm{para}}
\newcommand{\bN}{\mathcal{N}}
\newcommand{\oO}{\mathcal{O}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cm}{\mathcal{M}}
\newcommand{\ch}{\mathcal{H}}
\newcommand{\bigO}{\mathcal{O}} %
\newcommand{\cj}{\mathcal{J}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\CR}{\mathrm{CR}}
\newcommand{\noo}{\mathrm{no}}
\newcommand{\te}{\mathrm{te}}
\newcommand{\VC}{\mathrm{VC}}
\newcommand{\case}{\mathrm{case}}
\newcommand{\buu}{\mathbf{u}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\hP}{\mathbb{P}_n}
\newcommand{\hG}{\mathbb{G}}
\newcommand{\Op}{\mathrm{O}_{p}}
\newcommand{\op}{\mathrm{o}_{p}}
\newcommand{\Pa}{\mathrm{Pa}}
\newcommand{\pa}{\mathrm{\pa}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\calh}{\mathcal{H}}
\newcommand{\rI}{\mathrm{I}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\var}{\mathrm{var}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\rE}{\mathrm{E}}
\newcommand{\thpol}{\pi^{\theta}}
\newcommand{\thhatpol}{\pi^{\hat{\theta}}}
\newcommand{\rvar}{\mathrm{var}}
\newcommand{\Asmse}{\mathrm{Asmse}}
\newcommand{\dml}{\mathrm{dml}}
\newcommand{\dm}{\mathrm{dm}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\prns}[1]{\left(#1\right)}
\newcommand{\braces}[1]{\left\{#1\right\}}
\newcommand{\bracks}[1]{\left[#1\right]}
\newcommand{\sumT}{\sum_{t=0}^T}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\Rl}{\mathbb{R}}
\newcommand{\epol}{\pi^\mathrm{e}}
\newcommand{\bpol}{\pi^\mathrm{b}}
\newcommand{\pre}{\mathrm{pre}}
\newcommand{\tmle}{\mathrm{tmle}}
\newcommand{\ipw}{\mathrm{ipw}}
\newcommand{\prepi}[1]{d_0 \times #1}
\newcommand{\ini}{p_{\mathrm{ini}}}
\newcommand{\opera}{p_{\mathrm{op}}}
\newcommand{\inipi}[1]{p_{\mathrm{ini}, #1}}
\newcommand{\magd}[1]{\left\|#1\right\|}

\newcommand{\Rfrak}{\mathfrak{R}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Zcal}{\mathcal{Z}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\Lcal}{\mathcal{L}}

% Macros for the MWQL paper
\newcommand{\Lw}{L_{\mathrm{w}}}
\newcommand{\Lwn}{L_{\mathrm{w},n}}
\newcommand{\Lq}{L_{\mathrm{q}}}
\newcommand{\Lqn}{L_{\mathrm{q},n}}
\newcommand{\hatw}{\hat{w}}
\newcommand{\hatwn}{\hat{w}_n}
\newcommand{\hatq}{\hat{q}}
\newcommand{\hatqn}{\hat{q}_n}
\newcommand{\Rw}{R_{\mathrm{w}}}
\newcommand{\Rwn}{R_{\mathrm{w},n}}
\newcommand{\Rq}{R_{\mathrm{q}}}

\renewcommand{\eqref}[1]{(\ref{#1})}

\newcommand{\bepsilon}{{\mbox{\boldmath$\epsilon$}}}
\newcommand{\RN}[1]{%
  \textup{\uppercase\expandafter{\romannumeral#1}}%
}
\newcommand{\bmu}{{\mbox{\boldmath$\mu$}}}

\newcommand{\bbeta}{{\mbox{\boldmath$\beta$}}}

\newcount\Comments  % 0 suppresses notes to selves in text
\Comments=1 % TODO: change to 0 for final version

\def \x {\bm{x}}
\def \positiveData {{\{\bm{x}_i\}_{i=1}^{n}}}
\def \unlabeledData {{\{\bm{x}'_i\}_{i=1}^{n'}}}
\def \Rpositive {{\mathbb{R}^{+}}}
\def \hf {\hat{f}}
\def \hr {\hat{r}}
\def \htheta {\hat{\theta}}
\def \fstar {f^*}
\def \rstar {r^*}
\def \thetapi {{\theta_\pi}}
\def \hthetapi {{\hat{\theta}_\pi}}
\def \mysign {{\tt sign}}
\def \RPUB {{R^{\tt bias}_{\tt PU}}}
%\def \hfPU {\hf_{\mathrm{PU}}}
%\def \hfnnPU {\hf_{\mathrm{nnPU}}}
\def \hfPU {\hf_{1}}
\def \hfnnPU {\hf_{2}}
\def \dx {{\mathrm{d}\bm{x}}}
%\def \LagrangeMultiplierBeta {{\beta^*(\x)}}
%\def \LagrangeMultiplierAlpha {{\alpha^*(\x)}}
\def \LagrangeMultiplierBeta {{\mu}}
\def \LagrangeMultiplierAlpha {{\lambda}}
\def \iid {\overset{\mathrm{i.i.d.}}{\sim}}
\def \DOne {D_1}
\def \DTwo {D_2}
\def \Reg {\mathcal{R}}

%% Old notation
%\def \Risk {\mathcal{L}}
%\def \Emarginal {\mathbb{E}_{p_m}}
%\def \Emixture {\mathbb{E}_{p_m}}
%\def \du {\mathrm{d}u}
%\def \dx {\mathrm{d}x}
%\def \etamin {\eta_{\mathrm{min}}}
%\def \etamax {\eta_{\mathrm{max}}}
%\def \psimin {\psi_{\mathrm{min}}}
%\def \psimax {\psi_{\mathrm{max}}}
%\def \rmax {r_{\mathrm{max}}}
%\def \rmin {r_{\mathrm{min}}}

%%%% Teshima
%% Utility
\newcommand{\annot}[2]{\underbrace{#1}_{\text{#2}}}
\newcommand{\annotmath}[2]{\underbrace{#1}_{#2}}
%\newtheorem{definition}{Definition}

%% Base notation
\def \Re {\mathbb{R}}
\def \Na {\mathbb{N}}
\def \du {\mathrm{d}u}
%\def \dx {\mathrm{d}x}
\def \r {r}
\def \Ltwo {L^2}
\def \ltwo {\ell_2}
\newcommand \Probability[1]{\mathbb{P}\left(#1\right)}
\def \hE {\hat{\E}}
% Generic variables
\def \F {\mathcal{F}}
\def \G {\mathcal{G}}
\def \f {f}
\def \g {g}
\def \supf {\sup_{\f \in \F}}
\def \supg {\sup_{\g \in \G}}

%% Loss function etc.
\def \loss {\ell}
\newcommand{\br}{f} % Bregman divergence potential
%\def \br {\phi} % Bregman divergence potential
\def \tbr {\tilde\br}
\def \dbr {\partial \br}
\def \lossOne {\loss_1}
\def \lossTwo {\loss_2}
\def \LossBound {{B_\loss}}
\def \Cons {C}
%% \newcommand \modFn[1]{\left(#1\right)_+} % Modification function
% \newcommand \argmin[1]{\mathop{\rm arg~min}\limits_{#1}}
\def \modFn{\rho} % Modification function
%\def \rClass {\mathcal{H}_\r}
\newcommand{\rClass}{\mathcal{H}}
\newcommand{\rClassBound}{B_r}
\newcommand{\rClassBoundMin}{b_r}
\newcommand{\rClassRangeTwo}{(\rClassBoundMin, \rClassBound)}
\newcommand{\rClassRangeTwoName}{I_r}
\newcommand{\rClassRange}{(0, \rClassBound)}
\def \rClassRangeCl {[0, \rClassBound]}
\def \supr {\sup_{\r \in \rClass}}
\def \supt {\sup_{t \in \rClassRangeTwoName}}

%% Distributions and Data notation
% Distribution
\def \pnu {p_{\mathrm{nu}}}
\def \pde {p_{\mathrm{de}}}
\def \pmod {p_{\mathrm{mod}}}
%\def \rmax {r_{\mathrm{max}}}
\newcommand{\rmax}{\overline{R}}
\def \rmin {r_{\mathrm{min}}}
% Expectation
\def \Emarginal {\E_{p_m}}
\def \Emixture {\E_{p_m}}
\def \Enu {\E_{\mathrm{nu}}}
\def \Ede {\E_{\mathrm{de}}}
\def \Emod {\EX\hEmod} % Modified distribution p_de - C p_nu
%% \def \Emod {\E_{\mathrm{mod}}} % Modified distribution p_de - C p_nu
% Data
\def \nde {n_{\mathrm{de}}}
\def \nnu {n_{\mathrm{nu}}}
\def \hEnu {\hat{\E}_{\mathrm{nu}}}
\def \hEde {\hat{\E}_{\mathrm{de}}}
\def \hEmod {\hat{\E}_{\mathrm{mod}}}
% Risk
% \def \Risk {\mathcal{L}}
% \def \hRisk {\hat{\Risk}}
% \def \nnhRisk {\hRisk_{\mathrm{nn}}}
% \def \EnnhRisk {\E\nnhRisk}
\newcommand{\Risk}{\mathrm{BD}_{\br}}
\newcommand{\hRisk}{\widehat{\mathrm{BD}}_{\br}}
\newcommand{\nnhRisk}{\widehat{\mathrm{nnBD}}_{\br}}
\newcommand{\EnnhRisk}{\E\nnhRisk}


% Estimators and estimands
\def \rstar {r^*}
\def \rbest {\bar{r}}
\def \hr {\hat{\r}}

%% Theory 1: Estimation error bound
\def \Rad {\mathfrak{R}}
\def \Radmod {\Rad_{\mathrm{mod}}}
\newcommand{\Rademacher}[2]{\mathfrak{R}_{#1}^{#2}}
\newcommand{\Radnu}{\Rademacher{\nnu}{\pnu}}
\newcommand{\Radde}{\Rademacher{\nde}{\pde}}
\def \hERadnu {\hat{\E}^{\rad}_{\mathrm{nu}}}
\def \hERadde {\hat{\E}^{\rad}_{\mathrm{de}}}
\def \hERadmod {\hat{\E}^{\rad}_{\mathrm{mod}}}
\def \LipmodFn {L_\modFn}
\def \LipOne {L_{\lossOne}}
\def \LipTwo {L_{\lossTwo}}

%% Rademacher complexity
\def \rad {\sigma}
\def \ERad {\E_{\rad}}
\def \Rad {\mathcal{R}}

%% Symmetrization lemma
\def \EX {\E}
\def \EXjk {\EX_{(j, k)}}
\def \ghostMark {(\mathrm{gh})}
\def \EXghost {\E^{\ghostMark}}
\def \hEjk {\hE_{(i, j)}}
\def \hEghost {\hat{\E}^{\ghostMark}}
\def \hEghostjk {\hEghost_{(j, k)}}
\def \X {X}
\def \Xghost {X^{\ghostMark}}
\def \hS {\hat{S}}
\def \EhS {S}
\def \ljk {\loss_{(j, k)}}
\def \sumj {\sum_{j=1}^J}
\def \sumjk {\sum_{k=1}^{K_j}}
\def \Liprhoj {L_{\rho_j}}
\def \LipLossjk {L_{\ljk}}
\def \Radjk {\Rad_{\njk, \pjk}}
\def \hEXRad {\hE^{\rad}}
\def \hEXRadjk {\hEXRad_{(j, k)}}
\def \Indjk {\mathcal{I}_{(j, k)}}
\def \njk {n_{(j, k)}}
\def \pjk {p_{(j, k)}}
\def \InSpace {\mathcal{X}}
\def \FnSpace {\mathbb{R}^\InSpace}
\def \Xsetjk {\mathcal{D}_{(j, k)}}
% \def \Xsetjk {\InSpace_{(j, k)}}

%% Bias lemma
\newcommand \Indicator[1]{\mathbbm{1}\{#1\}}
\def \Identity {\mathrm{Id}}
\def \supp {\mathrm{supp}}
\def \modFnIdSupp {\supp(\modFn - \Identity)}
\def \modFnIdLip {L_{\modFn - \Identity}}
\def \infr {\inf_{\r \in \rClass}}
\newcommand{\lOneR}{\lossOne(\r(X))}
\def \modFnIdSet {\{t: \modFn(t) = t\}}
\newcommand{\BiasTerm}{\Phi_{(\Cons, \br, \modFn)}(\nnu, \nde)}
\newcommand{\BiasTermMainText}{\Phi_{\Cons}^\br(\nnu, \nde)}
\def \supLossVal {\sup_{s: |s| \leq (1+\Cons)\LossBound}}

%% Rademacher complexity bound
\def \InputBound {B_p}
\def \ParamBoundj {B_{W_j}}
\newcommand{\Radnp}{\Rademacher{n}{p}}
\def \rInnerClass {\mathcal{H}_f}
\def \dmax {d_{\mathrm{max}}}
\def \E {\mathbb{E}}

\newcommand{\lTwoR}{\lossTwo(\r(X))}
\newcommand{\lOne}[1]{\lossOne^{#1}}
\newcommand{\lTwo}[1]{\lossTwo^{#1}}
\newcommand{\lzeroNrm}[1]{\|#1\|_0}
\newcommand{\hEmodTwo}{\hEmod'}
\newcommand{\nnuz}{\nnu^0}
\newcommand{\ndez}{\nde^0}
\newcommand{\AppdxEmpProcMcDiarmidRadSum}{\mathcal{R}}
\newcommand{\smallO}{
  \mathchoice
  {{\scriptstyle\mathcal{O}}}% \displaystyle
  {{\scriptstyle\mathcal{O}}}% \textstyle
  {{\scriptscriptstyle\mathcal{O}}}% \scriptstyle
  {\scalebox{.6}{$\scriptscriptstyle\mathcal{O}$}}%\scriptscriptstyle
}
% \newcommand{\bigO}{\mathcal{O}}
\newcommand{\order}{\smallO{}}
\newcommand{\Order}[1]{\bigO\left(#1\right)}
\newcommand{\orderp}{\smallO{}_{\mathbb{P}}}
\newcommand{\Orderp}[1]{\bigO_{p}\left(#1\right)}
\newcommand{\sparseNetworkRadBoundConst}{c}
\newcommand{\Lmax}{\bar{L}}
\newcommand{\pmax}{\bar{p}}
\newcommand{\rClassMconditionSet}{\mathrm{cond}_M}
\newcommand{\rClassM}{\rClass_M}
\newcommand{\bracketEntropy}[3]{\log \mathcal{N}\left(#1, #2, #3\right)}
\newcommand{\coveringNumber}[3]{\mathcal{N}\left(#1, #2, #3\right)}
\newcommand{\inftyCoveringNumber}[2]{\coveringNumber{#1}{#2}{\|\cdot\|_\infty}}
\newcommand{\rClassMSupNormBoundConst}{c_0}
\newcommand{\rClassMLpNormBoundConst}{c_1}
\newcommand{\disjointUnion}{\coprod}
\newcommand{\IndLP}{\mathrm{Ind}_{\Lmax,\pmax}}
\newcommand{\IndLPM}{\stackrel{(L, p) \in \IndLP}{I_1(L, p) \leq M}}
\newcommand{\IndLPMInline}{(L, p) \in \IndLP: I_1(L, p) \leq M}
\newcommand{\rClassLP}{\rClass(L, p, s, F)}
\newcommand{\elled}[1]{\ell \circ #1}
\newcommand{\ellLip}{\nu}
% \newcommand{\vmax}[2]{#1 \vee #2}
% \newcommand{\vmin}[2]{#1 \wedge #2}
\newcommand{\vmax}[2]{\max\left\{#1, #2\right\}}
\newcommand{\vmin}[2]{\min\left\{#1, #2\right\}}
\newcommand{\exponentialOrderOne}{\exp\left(- \frac{2 \alpha^2}{(\LossBound^2/\nde) + (\Cons^2\LossBound^2 / \nnu)}\right)}


==> IWMM (1)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

